Cost-Aware Automatic Program Repair

We present a formal framework for repairing infinite-state, imperative, sequential programs, with (possibly recursive) procedures and multiple assertions; the framework can generate repaired programs by modifying the original erroneous program in multiple program locations, and can ensure the readability of the repaired program using user-defined expression templates; the framework also generates a set of inductive assertions that serve as a proof of correctness of the repaired program. As a step toward integrating programmer intent and intuition in automated program repair, we present a " cost-aware" formulation - given a cost function associated with permissible statement modifications, the goal is to ensure that the total program modification cost does not exceed a given repair budget. As part of our predicate abstraction-based solution framework, we present a sound and complete algorithm for repair of Boolean programs. We have developed a prototype tool based on SMT solving and used it successfully to repair diverse errors in benchmark C programs.

==> Figures/ex4.tex <==

\begin{figure}[h]
\centering
\scalebox{0.8}{
\fbox{
\begin{minipage}{0.55\linewidth}
\footnotesize{
{\tt
%$\mtt{necex14}:$\\
%\\
int main() $\{$\\
\hspace*{3mm} int $x,y$;\\
\hspace*{3mm} int $a[10]$;\\
\hspace*{3mm} $\ell_1:$ $x \; \assign \; 1U$;\\
\hspace*{3mm} $\ell_2:$ while ($x \leq 10U$) $\{$\\
\hspace*{3mm} $\ell_3:$ \hspace*{3mm} $y \; \assign \; 11-x$;\\
\hspace*{3mm} $\ell_4:$ \hspace*{3mm} assert ($y \geq 0 \; \wedge \;
y<10$);\\
\hspace*{3mm} $\ell_5:$ \hspace*{3mm} $a[y] \; \assign \; -1$;\\
\hspace*{3mm} $\ell_6:$ \hspace*{3mm} $x \; \assign \; x + 1$;\\
\hspace*{9mm} $\}$\\
$\}$\\
}}
\end{minipage}
%\noindent\rule{8.5cm}{0.4pt}
%\\
\begin{minipage}{0.5\linewidth}
\footnotesize{
{\bf Boolean program vars/predicates:}\\
%\begin{enumerate}
$\conc(b_0) \; =  \; y < 0 $, 
$\conc(b_1) \; =  \; y < 10 $\\
%\end{enumerate}
\noindent\rule{4.7cm}{0.4pt}
\\
{\bf Boolean program repair:}\\
%\begin{enumerate}
Change $stmt(\ell_3)$ from \\ 
$b_0,b_1 \; \assign \; *,*$ to 
$b_0,b_1 \; \assign \; \mtt{F},\mtt{T}$\\
%\end{enumerate}
\noindent\rule{4.7cm}{0.4pt}
\\
{\bf Concrete program repair:}\\
%\begin{enumerate}
Change $stmt(\ell_3)$ to $y \; \assign \; 10 - x$\\
%\end{enumerate}
\noindent\rule{4.7cm}{0.4pt}
\\
{\bf Inductive Assertions:}\\
%\begin{enumerate}
They were all $true$
%\end{enumerate}
}
\end{minipage}
}
}
\caption{Repairing program $\mtt{necex14}$}
\label{fig:ex4}
\end{figure}



==> Figures/syntax.tex <==
\begin{figure}
\footnotesize{
\begin{center}
\begin{tabular}[t]{|p{1.2cm}lp{5.6cm}|}
\hline
$\en{pgm}$ & $::=$ & $\en{vardecl} \, \en{proclist}$\\
$\en{vardecl}$ & $::=$ & $\mtt{decl} \; \varname :  \en{type} \bm{;}$ $|$
$\en{vardecl} \, \en{vardecl}$\\

$\en{proclist}$ & $::=$ & $\en{proc} \, \en{proclist}$ $|$ $\en{proc}$\\

$\en{proc}$ & $::=$ & $\f(\varname_1,\ldots,\varname_\formalind) \, \mtt{begin} \, \en{vardecl}
\, \en{stmtseq} \, \mtt{end}$\\

$\en{stmtseq}$ & $::=$ & $\en{labstmt} \, \bm{;} \, \en{stmtseq}$\\

$\en{labstmt}$ & $::=$ & $\en{stmt}$ $|$ $\ell: \en{stmt}$\\

$\en{stmt}$ & $::=$ & $\varname_1,\ldots, \varname_\assind \, \bm{\assign} \, \en{expr_1},\ldots,\en{expr_m}$
\newline
$|$ $\mtt{assume} \, (\en{bexpr})$ $|$ $\mtt{assert} \,  (\en{bexpr})$
\newline
$|$ $\mtt{call} \; \f(\en{expr_1},\ldots,\en{expr_\formalind})$
$|$ $\mtt{return}$
\newline
$|$ $\mtt{goto} \; \ell_1\, \mtt{or} \ldots \mtt{or}\, \ell_n$ $|$ $\mtt{skip}$\\

$\en{bexpr}$ & $::=$ & $*$ $|$ $\true$ $|$ $\false$ $|$ $\var$ $|$ 
$\neg\en{bexpr}$ 
\newline 
$|$ $\en{bexpr} \vee \en{bexpr}$ $|$ 
$\en{bexpr} \wedge \en{bexpr}$ 
\newline
$|$ $\en{bexpr} \Rightarrow \en{bexpr}$ 
$|$ $\en{bexpr} = \en{bexpr}$ 
\newline
$|$ $\en{bexpr} \neq \en{bexpr}$\\
%$\mtt{choose}(\en{bexpr},\en{bexpr})$\\
\hline
\end{tabular}
\end{center}
}
\caption{Programming language syntax}
\label{fig:syntax}
\end{figure}

